Revisiting Computational Storage for Data Integrity and Security

The idea of computational storage device (CSD) has come a long way since at least 1990s [1], [2]. By embedding computing resources within storage devices, CSDs could potentially offload computational tasks from CPUs and enable near-data processing (NDP), reducing data movements and/or energy consumption significantly. While the initial hard-disk-based CSDs suffer from severe limitations in terms of on-drive resources, programmability, etc., the storage market has witnessed the commercialization of solid-state-drive (SSD) based CSDs (e.g., Samsung SmartSSD [3], ScaleFlux CSDs [4]) recently, which has enabled CSD-based optimizations for avariety of application scenarios (e.g., [5], [6], [7]).

==> reference.tex <==
@inproceedings{panda-dolan2015repeatable,
  title={Repeatable reverse engineering with PANDA},
  author={Dolan-Gavitt, Brendan and Hodosh, Josh and Hulin, Patrick and Leek, Tim and Whelan, Ryan},
  booktitle={Proceedings of the 5th Program Protection and Reverse Engineering Workshop},
  year={2015}
}

@inproceedings{vinter-atc22,
  title={Vinter: Automatic Non-Volatile Memory Crash Consistency Testing for Full Systems},
  author={Samuel Kalbfleisch and Lukas Werling and Frank Bellosa},
  booktitle={Proceedings of the 2022 USENIX Annual Technical Conference},
  year={2022}
}

@inproceedings{chipmunk-eurosys23,
  title={Chipmunk: Investigating Crash-Consistency in Persistent-Memory File Systems},
  author={Hayley LeBlanc and Shankara Pailoor and Om Saran K R E and Isil Dillig and James Bornholt and Vijay Chidambaram},
  booktitle={Proceedings of the Eightteenth European Conference on Computer Systems},
  year={2023}
}

@misc{Pmem-Redis,
	title = {Pmem-Redis },
	howpublished = "\url{https://github.com/pmem/pmem-redis}",
	year = {2021},
}

@misc{patch,
	title = {blkdev: flush disk cache on ->fsync },
	howpublished = "\url{https://git.kernel.org/pub/scm/linux/kernel/git/stable/linux.git/commit/?id=ab0a9735e06914ce4d2a94ffa41497dbc142fe7f}",
	
}

@inproceedings{pmprogram,
  title={Introduction to Persistent Memory Programming},
  author={Samuel Kalbfleisch and Lukas Werling and Frank Bellosa},
  booktitle={ Programming Persistent Memory: A Comprehensive Guide for Developers},
  year={2020}
}
@inproceedings{icde2018,
  title={An NVM Carol: Visions of NVM Past, Present, and Future},
  author={Margo Seltzer and Virendra Marathe and Steve Byan},
  booktitle={2018 IEEE 34th International Conference
on Data Engineering (ICDE)},
  year={2018}
}
@inproceedings{fast20,
  title={An Empirical Guide
to the Behavior and Use of Scalable Persistent Memory},
  author={Jian Yang and Juno Kim and Morteza Hoseinzadeh and Joseph Izraelevitz and Steve Swanson},
  booktitle={Proceedings of 18th USENIX Conference on File and Storage
Technologies},
  year={2020}
}

@misc{pm,
	title = {What is Persistent Memory? },
	howpublished = "\url{https://www.snia.org/education/what-is-persistent-memory}",
	
}

@misc{pmfs,
	title = {PMFS Introduction },
	howpublished = "\url{https://github.com/linux-pmfs/pmfs}",
	
}

@misc{ext4dax,
	title = {Enable ext4 support for per-file/directory DAX operations},
	howpublished = "\url{https://lwn.net/Articles/817444/}",
	
}

@inproceedings{nova,
  title={NOVA: A Log-structured File System for Hybrid Volatile/Non-volatile Main Memories},
  author={Jian Xu and Steven Swanson},
  booktitle={Proceedings of 14th USENIX Conference on File and Storage
Technologies},
  year={2016}
}

@misc{pmdk,
	title = {Persistent Memory Development Kits},
	howpublished = "\url{https://pmem.io/pmdk/}",
	
}

@inproceedings{apsys17,
  title={Programming for Non-Volatile Main Memory Is Hard},
  author={Jinglei Ren and Qingda Hu and Samira Khan and Thomas Moscibroda},
  booktitle={Proceedings of the 8th Asia Pacific Workshop on Systems},
  year={2017}
}
@inproceedings{Jeremysosp09,
  title={Better I/O through byte-addressable, persistent memory},
  author={Jeremy Condit and Edmund B. Nightingale and Christopher Frost and Engin
Ipek and Benjamin Lee and Doug Burger and Derrick Coetzee},
  booktitle={Proceedings of the
ACM SIGOPS 22nd Symposium on Operating Systems Principles},
  year={2009}
}
@misc{cxl,
	title = {Compute Express Link},
	howpublished = "\url{https://www.computeexpresslink.org/}",
	
}

@inproceedings{bhardwaj2022cache,
  title={Cache-coherent accelerators for persistent memory crash consistency},
  author={Ankit Bhardwaj and Todd Thornley and Vinita Pawar and Reto Achermann and Gerd Zellweger and Ryan Stutsman
},
  booktitle={Proceedings of the 14th ACM Workshop on Hot Topics in Storage and File Systems},
  year={2022}
}

@misc{intel-pmemio-update,
	title = {UPDATE ON PMDK AND OUR LONG TERM SUPPORT STRATEGY},
	howpublished = "\url{https://pmem.io/blog/2022/11/update-on-pmdk-and-our-long-term-support-strategy/}",	
}

@inproceedings{SYSTOR21-Duo,
  title={A study of persistent memory bugs in the Linux kernel},
  author={Duo Zhang and Om Rameshwar Gatla and Wei Xu and Mai Zheng},
  booktitle={Proceedings of the 14th ACM International Conference on Systems and Storage},
  year={2021}
}

@inproceedings{crashmonkey-hotstor17,
  title={{CrashMonkey: A Framework to Systematically Test File-System Crash Consistency}},
  author={Martinez, Ashlie and Chidambaram, Vijay},
  booktitle={{Proceedings of the 9th USENIX Conference on Hot Topics in Storage and File Systems (HotStorage)}},
  year={2017}
}

@inproceedings{vjay-osdi18-blackboxtesting,
  title={Finding crash-consistency bugs with bounded black-box crash testing},
  author={Mohan, Jayashree and Martinez, Ashlie and Ponnapalli, Soujanya and Raju, Pandian and Chidambaram, Vijay},
  booktitle={13th $\{$USENIX$\}$ Symposium on Operating Systems Design and Implementation ($\{$OSDI$\}$ 18)},
  pages={33--50},
  year={2018}
}

@InProceedings{ChidambaramEtAl13-OptFS,
	title = "{Optimistic Crash Consistency}",
	author = "Vijay Chidambaram and Thanumalayan Sankaranarayana Pillai and Andrea C. Arpaci-Dusseau and Remzi H. Arpaci-Dusseau",
	booktitle = "Proceedings of the 24th ACM Symposium on Operating Systems Principles (SOSP '13)",
	month = "November",
	year = "2013",
	address    = "Farmington, PA",
}

@inproceedings{sigurbjarnarson2016push,
	title={Push-button verification of file systems via crash refinement},
	author={Sigurbjarnarson, Helgi and Bornholt, James and Torlak, Emina and Wang, Xi},
	booktitle={Proceedings of 12th USENIX Symposium on Operating Systems Design and Implementation (OSDI'16)},
	year={2016},
}

@inproceedings {Om-FAST18-RFSCK,
	author = {Om Rameshwar Gatla and Muhammad Hameed and Mai Zheng and Viacheslav Dubeyko and Adam Manzanares and Filip Blagojevi{\'c} and Cyril Guyot and Robert Mateescu},
	title = {Towards Robust File System Checkers},
	booktitle = {Proceedings of the 16th {USENIX} Conference on File and Storage Technologies ({FAST})},
	year = {2018},
}

@inproceedings{Zheng-OSDI14-DB,
	author = {Mai Zheng and Joseph Tucek and Dachuan Huang and Feng Qin and Mark Lillibridge and Elizabeth S. Yang and Bill W Zhao and Shashank Singh},
	title = {{Torturing Databases for Fun and Profit}},
	booktitle = {11th USENIX Symposium on Operating Systems Design and Implementation (OSDI 14)},
	year = {2014},
	isbn = { 978-1-931971-16-4},
	pages = {449--464},
}


@inproceedings{Octopus-atc17,
  title={Octopus+: An RDMA-Enabled Distributed Persistent Memory File System},
  author={Bohong Zhu and Youmin Chen and Qing Wang and Youyou Lu and Jiwu Shu},
  booktitle={ACM Transactions on Storage},
  year={2021}
}

@inproceedings{FIRM-micro14,
  title={FIRM: Fair and High-Performance Memory Control for Persistent Memory Systems},
  author={Jishen Zhao and Onur Mutlu and Yuan Xie},
  booktitle={47th Annual IEEE/ACM International Symposium on Microarchitecture},
  year={2014}
},


@misc{xilinx,
    title = "{P2P bandwidth Example}",
    author = "{Xilinx}",
    howpublished = "\url{https://github.com/Xilinx/Vitis_Accel_Examples/tree/2022.2/host/p2p_bandwidth}",
    note = "Accessed: 2024-03-25"
},

@inproceedings{adams2021enabling,
  title={Enabling near-data processing in distributed object storage systems},
  author={Adams, Ian F and Agrawal, Neha and Mesnier, Michael P},
  booktitle={Proceedings of the 13th ACM Workshop on Hot Topics in Storage and File Systems},
  pages={28--34},
  year={2021}
},

@misc{standard,
    title = "{Computational Storage Architecture and Programming Model v1.0}",
    author ="{SNIA}",
    howpublished = "\url{https://www.snia.org/sites/default/files/technical-work/computational/release/SNIA-Computational-Storage-Architecture-and-Programming-Model-1.0.pdf}",
    note = "Accessed: 2022-08-30"
},

@misc{ceph-jerasure,
    title = "{Jerasure plugin - Ceph Documentation}",
    howpublished = "\url{https://docs.ceph.com/en/pacific/dev/osd_internals/erasure_coding/jerasure/}",
    note = "Accessed: 2024-03-29"
},

@inproceedings{fault-tolerance-kolosov,
    author = "Itzhak Kolosov AND others",
    title = "{On Fault Tolerance, Locality, and Optimality in Locally Repairable Codes}",
    booktitle = "{Proceedings of the 2018 USENIX Annual Technical Conference}",
    pages = 870,
    year = 2018
},

@inproceedings{silberstein2014lazy,
  title={Lazy means smart: Reducing repair bandwidth costs in erasure-coded distributed storage},
  author={Silberstein, Mark and Ganesh, Lakshmi and Wang, Yang and Alvisi, Lorenzo and Dahlin, Mike},
  booktitle={Proceedings of International Conference on Systems and Storage},
  pages={1--7},
  year={2014}
},

@article{plank2008jerasure,
  title={Jerasure: A library in C/C++ facilitating erasure coding for storage applications-Version 1.2},
  author={Plank, James S and Simmerman, Scott and Schuman, Catherine D},
  journal={University of Tennessee, Tech. Rep. CS-08-627},
  volume={23},
  year={2008}
},

@ARTICLE{edgecomputing,
  author={Liang, Lixin and He, Huan and Zhao, Jian and Liu, Chengjian and Luo, Qiuming and Chu, Xiaowen},
  journal={IEEE Access}, 
  title={An Erasure-Coded Storage System for Edge Computing}, 
  year={2020},
  volume={8},
  number={},
  pages={96271-96283},
  keywords={Encoding;Edge computing;Performance evaluation;Cloud computing;Bandwidth;Data centers;Decoding;Erasure-coded storage system;edge computing;erasure coding;jetson nano},
  doi={10.1109/ACCESS.2020.2995973}},

@ARTICLE{networkaccelerate,
  author={Qiao, Yi and Zhang, Menghao and Zhou, Yu and Kong, Xiao and Zhang, Han and Xu, Mingwei and Bi, Jun and Wang, Jilong},
  journal={IEEE Transactions on Parallel and Distributed Systems}, 
  title={NetEC: Accelerating Erasure Coding Reconstruction With In-Network Aggregation}, 
  year={2022},
  volume={33},
  number={10},
  pages={2571-2583},
  keywords={Encoding;Decoding;Codes;Throughput;Task analysis;Switches;Bandwidth;Erasure coding;distributed storage sytems;programmable switch;software-defined networks},
  doi={10.1109/TPDS.2022.3145836}},

@inproceedings{do2013query,
  title={Query processing on smart ssds: Opportunities and challenges},
  author={Do, Jaeyoung and Kee, Yang-Suk and Patel, Jignesh M and Park, Chanik and Park, Kwanghyun and DeWitt, David J},
  booktitle={Proceedings of the 2013 ACM SIGMOD International Conference on Management of Data},
  pages={1221--1230},
  year={2013}
},

@article{kim2021understanding,
  title={Understanding the Performance Characteristics of Computational Storage Drives: A Case Study with SmartSSD},
  author={Kim, Hwajung and Yeom, Heon Y and Sung, Hanul},
  journal={Electronics},
  volume={10},
  number={21},
  pages={2617},
  year={2021},
  publisher={MDPI}
},

@inproceedings{salamat2021nascent,
  title={NASCENT: Near-storage acceleration of database sort on SmartSSD},
  author={Salamat, Sahand and Haj Aboutalebi, Armin and Khaleghi, Behnam and Lee, Joo Hwan and Ki, Yang Seok and Rosing, Tajana},
  booktitle={The 2021 ACM/SIGDA International Symposium on Field-Programmable Gate Arrays},
  pages={262--272},
  year={2021}
},

@inproceedings{silberstein2014lazy,
  title={Lazy means smart: Reducing repair bandwidth costs in erasure-coded distributed storage},
  author={Silberstein, Mark and Ganesh, Lakshmi and Wang, Yang and Alvisi, Lorenzo and Dahlin, Mike},
  booktitle={Proceedings of International Conference on Systems and Storage},
  pages={1--7},
  year={2014}
},

@article{luby2019liquid,
  title={Liquid cloud storage},
  author={Luby, Michael and Padovani, Roberto and Richardson, Thomas J and Minder, Lorenz and Aggarwal, Pooja},
  journal={ACM Transactions on Storage (TOS)},
  volume={15},
  number={1},
  pages={1--49},
  year={2019},
  publisher={ACM New York, NY, USA}
},

@inproceedings{daoud2024peer,
  title={Peer-to-Peer Data Transfer Evaluation in SmartSSD-based Multi-devices System},
  author={Daoud, Luka and Sun, Gongjin and Huen, Hingkwan},
  booktitle={Proceedings of 36th International Conference on},
  volume={97},
  pages={72--80},
  year={2024}
},

@article{lee2020smartssd,
  title={SmartSSD: FPGA accelerated near-storage data analytics on SSD},
  author={Lee, Joo Hwan and Zhang, Hui and Lagrange, Veronica and Krishnamoorthy, Praveen and Zhao, Xiaodong and Ki, Yang Seok},
  journal={IEEE Computer architecture letters},
  volume={19},
  number={2},
  pages={110--113},
  year={2020},
  publisher={IEEE}
},

@article{Acharya-ActiveDisk-ASPLOS98,
author = {Acharya, Anurag and Uysal, Mustafa and Saltz, Joel},
title = {Active disks: programming model, algorithms and evaluation},
year = {1998},
issue_date = {Dec. 1998},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {32},
number = {5},
issn = {0163-5980},
url = {https://doi.org/10.1145/384265.291026},
doi = {10.1145/384265.291026},
abstract = {Several application and technology trends indicate that it might be both profitable and feasible to move computation closer to the data that it processes. In this paper, we evaluate Active Disk architectures which integrate significant processing power and memory into a disk drive and allow application-specific code to be downloaded and executed on the data that is being read from (written to) disk. The key idea is to offload bulk of the processing to the diskresident processors and to use the host processor primarily for coordination, scheduling and combination of results from individual disks. To program Active Disks, we propose a stream-based programming model which allows disklets to be executed efficiently and safely. Simulation results for a suite of six algorithms from three application domains (commercial data warehouses, image processing and satellite data processing) indicate that for these algorithms, Active Disks outperform conventional-disk architectures.},
journal = {SIGOPS Oper. Syst. Rev.},
month = {oct},
pages = {81–91},
numpages = {11}
},

@inproceedings{Riedel-ActiveStorage-VLDB98,
author = {Riedel, Erik and Gibson, Garth A. and Faloutsos, Christos},
title = {Active Storage for Large-Scale Data Mining and Multimedia},
year = {1998},
isbn = {1558605665},
publisher = {Morgan Kaufmann Publishers Inc.},
address = {San Francisco, CA, USA},
booktitle = {Proceedings of the 24rd International Conference on Very Large Data Bases},
pages = {62–73},
numpages = {12},
series = {VLDB '98}
},

@inproceedings{Cao-POLARDB-FAST20,
author = {Cao, Wei and Zhang, Yingqiang and Yang, Xinjun and Li, Feifei and Wang, Sheng and Hu, Qingda and Cheng, Xuntao and Chen, Zongzhi and Liu, Zhenjun and Fang, Jing and Wang, Bo and Wang, Yuhui and Sun, Haiqing and Yang, Ze and Cheng, Zhushi and Chen, Sen and Wu, Jian and Hu, Wei and Zhao, Jianwei and Gao, Yusong and Cai, Songlu and Zhang, Yunyang and Tong, Jiawang},
title = {PolarDB Serverless: A Cloud Native Database for Disaggregated Data Centers},
year = {2021},
isbn = {9781450383431},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3448016.3457560},
doi = {10.1145/3448016.3457560},
abstract = {beginabstract The trend in the DBMS market is to migrate to the cloud for elasticity, high availability, and lower costs. The traditional, monolithic database architecture is difficult to meet these requirements. With the development of high-speed network and new memory technologies, disaggregated data center has become a reality: it decouples various components from monolithic servers into separated resource pools (e.g., compute, memory, and storage) and connects them through a high-speed network. The next generation cloud native databases should be designed for disaggregated data centers. In this paper, we describe the novel architecture of name, which follows thedisaggregation design paradigm: the CPU resource on compute nodes is decoupled from remote memory pool and storage pool. Each resource pool grows or shrinks independently, providing revon-demand provisoning at multiple dimensions while improving reliability. We also design our system to mitigate the inherent penalty brought by resource disaggregation, and introduce optimizations such as optimistic locking and index awared prefetching. Compared to the architecture that uses local resources, name achieves better dynamic resource provisioning capabilities and 5.3 times faster failure recovery speed, while achieving comparable performance. endabstract},
booktitle = {Proceedings of the 2021 International Conference on Management of Data},
pages = {2477–2489},
numpages = {13},
keywords = {shared storage, shared remote memory, disaggregated data center, cloud database},
location = {Virtual Event, China},
series = {SIGMOD '21}
},

@inproceedings{Qiao-BTreeLSMTree-FAST22,
  title={Closing the B+-tree vs.$\{$LSM-tree$\}$ Write Amplification Gap on Modern Storage Hardware with Built-in Transparent Compression},
  author={Qiao, Yifan and Chen, Xubin and Zheng, Ning and Li, Jiangpeng and Liu, Yang and Zhang, Tong},
  booktitle={20th USENIX Conference on File and Storage Technologies (FAST 22)},
  pages={69--82},
  year={2022}
},

@misc{samsung-smartssd,
    title           = "Samsung SmartSSD",
    author          = "{AMD Xilinx}",
    howpublished    = "\url{https://www.xilinx.com/applications/data-center/computational-storage/smartssd.html}"   
},

@inproceedings{Remzi-IRON-FileSystem-SOSP05,
author = {Prabhakaran, Vijayan and Bairavasundaram, Lakshmi N. and Agrawal, Nitin and Gunawi, Haryadi S. and Arpaci-Dusseau, Andrea C. and Arpaci-Dusseau, Remzi H.},
title = {IRON file systems},
year = {2005},
isbn = {1595930795},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1095810.1095830},
doi = {10.1145/1095810.1095830},
abstract = {Commodity file systems trust disks to either work or fail completely, yet modern disks exhibit more complex failure modes. We suggest a new fail-partial failure model for disks, which incorporates realistic localized faults such as latent sector errors and block corruption. We then develop and apply a novel failure-policy fingerprinting framework, to investigate how commodity file systems react to a range of more realistic disk failures. We classify their failure policies in a new taxonomy that measures their Internal RObustNess (IRON), which includes both failure detection and recovery techniques. We show that commodity file system failure policies are often inconsistent, sometimes buggy, and generally inadequate in their ability to recover from partial disk failures. Finally, we design, implement, and evaluate a prototype IRON file system, Linux ixt3, showing that techniques such as in-disk checksumming, replication, and parity greatly enhance file system robustness while incurring minimal time and space overheads.},
booktitle = {Proceedings of the Twentieth ACM Symposium on Operating Systems Principles},
pages = {206–220},
numpages = {15},
keywords = {IRON file systems, block corruption, disks, fail-partial failure model, fault tolerance, internal, latent sector errors, redundancy, reliability, storage},
location = {Brighton, United Kingdom},
series = {SOSP '05}
},

@article{Om-TOS18,
author = {Gatla, Om Rameshwar and Zheng, Mai and Hameed, Muhammad and Dubeyko, Viacheslav and Manzanares, Adam and Blagojevic, Filip and Guyot, Cyril and Mateescu, Robert},
title = {Towards Robust File System Checkers},
year = {2018},
issue_date = {November 2018},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {14},
number = {4},
issn = {1553-3077},
url = {https://doi.org/10.1145/3281031},
doi = {10.1145/3281031},
abstract = {File systems may become corrupted for many reasons despite various protection techniques. Therefore, most file systems come with a checker to recover the file system to a consistent state. However, existing checkers are commonly assumed to be able to complete the repair without interruption, which may not be true in practice. In this work, we demonstrate via fault injection experiments that checkers of widely used file systems (EXT4, XFS, BtrFS, and F2FS) may leave the file system in an uncorrectable state if the repair procedure is interrupted unexpectedly. To address the problem, we first fix the ordering issue in the undo logging of e2fsck and then build a general logging library (i.e., rfsck-lib) for strengthening checkers. To demonstrate the practicality, we integrate rfsck-lib with existing checkers and create two new checkers: rfsck-ext, a robust checker for Ext-family file systems, and rfsck-xfs, a robust checker for XFS file systems, both of which require only tens of lines of modification to the original versions. Both rfsck-ext and rfsck-xfs are resilient to faults in our experiments. Also, both checkers incur reasonable performance overhead (i.e., up to 12\%) compared to the original unreliable versions. Moreover, rfsck-ext outperforms the patched e2fsck by up to nine times while achieving the same level of robustness.},
journal = {ACM Trans. Storage},
month = {dec},
articleno = {35},
numpages = {25},
keywords = {file-system faults, data corruption, Fault tolerance}
},

@inproceedings{Remzi-FAST17-RedundencyDoesNotImplyFaultTolerance,
author = {Ganesan, Aishwarya and Alagappan, Ramnatthan and Arpaci-Dusseau, Andrea C. and Arpaci-Dusseau, Remzi H.},
title = {Redundancy does not imply fault tolerance: analysis of distributed storage reactions to single errors and corruptions},
year = {2017},
isbn = {9781931971362},
publisher = {USENIX Association},
address = {USA},
abstract = {We analyze how modern distributed storage systems behave in the presence of file-system faults such as data corruption and read and write errors. We characterize eight popular distributed storage systems and uncover numerous bugs related to file-system fault tolerance. We find that modern distributed systems do not consistently use redundancy to recover from file-system faults: a single file-system fault can cause catastrophic outcomes such as data loss, corruption, and unavailability. Our results have implications for the design of next generation fault-tolerant distributed and cloud storage systems.},
booktitle = {Proceedings of the 15th Usenix Conference on File and Storage Technologies},
pages = {149–165},
numpages = {17},
location = {Santa clara, CA, USA},
series = {FAST'17}
},

@inproceedings{JinruiCao-ICS18-PFault,
author = {Cao, Jinrui and Gatla, Om Rameshwar and Zheng, Mai and Dai, Dong and Eswarappa, Vidya and Mu, Yan and Chen, Yong},
title = {PFault: A General Framework for Analyzing the Reliability of High-Performance Parallel File Systems},
year = {2018},
isbn = {9781450357838},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3205289.3205302},
doi = {10.1145/3205289.3205302},
abstract = {High-performance parallel file systems (PFSes) are of prime importance today. However, despite the importance, their reliability is much less studied compared with that of local storage systems, largely due to the lack of an effective analysis methodology.In this paper, we introduce PFault, a general framework for analyzing the failure handling of PFSes. PFault automatically emulates the failure state of each storage device in the target PFS based on a set of well-defined fault models, and enables analyzing the recoverability of the PFS under faults systematically.To demonstrate the practicality, we apply PFault to study Lustre, one of the most widely used PFSes. Our analysis reveals a number of cases where Lustre's checking and repairing utility LFSCK fails with unexpected symptoms (e.g., I/O error, hang, reboot). Moreover, with the help of PFault, we are able to identify a resource leak problem where a portion of Lustre's internal namespace and storage space become unusable even after running LFSCK. On the other hand, we also verify that the latest Lustre has made noticeable improvement in terms of failure handling comparing to a previous version. We hope our study and framework can help improve PFSes for reliable high-performance computing.},
booktitle = {Proceedings of the 2018 International Conference on Supercomputing},
pages = {1–11},
numpages = {11},
keywords = {Parallel file systems, high performance computing, reliability},
location = {Beijing, China},
series = {ICS '18}
},

@article{Runzhou-TOS22-StudyPFS,
author = {Han, Runzhou and Gatla, Om Rameshwar and Zheng, Mai and Cao, Jinrui and Zhang, Di and Dai, Dong and Chen, Yong and Cook, Jonathan},
title = {A Study of Failure Recovery and Logging of High-Performance Parallel File Systems},
year = {2022},
issue_date = {May 2022},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {18},
number = {2},
issn = {1553-3077},
url = {https://doi.org/10.1145/3483447},
doi = {10.1145/3483447},
abstract = {Large-scale parallel file systems (PFSs) play an essential role in high-performance computing (HPC). However, despite their importance, their reliability is much less studied or understood compared with that of local storage systems or cloud storage systems. Recent failure incidents at real HPC centers have exposed the latent defects in PFS clusters as well as the urgent need for a systematic analysis.To address the challenge, we perform a study of the failure recovery and logging mechanisms of PFSs in this article. First, to trigger the failure recovery and logging operations of the target PFS, we introduce a black-box fault injection tool called  PFault, which is transparent to PFSs and easy to deploy in practice.  PFault emulates the failure state of individual storage nodes in the PFS based on a set of pre-defined fault models and enables examining the PFS behavior under fault systematically.Next, we apply PFault to study two widely used PFSs: Lustre and BeeGFS. Our analysis reveals the unique failure recovery and logging patterns of the target PFSs and identifies multiple cases where the PFSs are imperfect in terms of failure handling. For example, Lustre includes a recovery component called LFSCK to detect and fix PFS-level inconsistencies, but we find that LFSCK itself may hang or trigger kernel panics when scanning a corrupted Lustre. Even after the recovery attempt of LFSCK, the subsequent workloads applied to Lustre may still behave abnormally (e.g., hang or report I/O errors). Similar issues have also been observed in BeeGFS and its recovery component BeeGFS-FSCK. We analyze the root causes of the abnormal symptoms observed in depth, which has led to a new patch set to be merged into the coming Lustre release. In addition, we characterize the extensive logs generated in the experiments in detail and identify the unique patterns and limitations of PFSs in terms of failure logging. We hope this study and the resulting tool and dataset can facilitate follow-up research in the communities and help improve PFSs for reliable high-performance computing.},
journal = {ACM Trans. Storage},
month = {apr},
articleno = {14},
numpages = {44},
keywords = {storage systems, high performance computing, logging, failure handling, reliability, file system checkers, Parallel file systems}
},

@INPROCEEDINGS{hdfs_msst10,
  author={Shvachko, Konstantin and Kuang, Hairong and Radia, Sanjay and Chansler, Robert},
  booktitle={2010 IEEE 26th Symposium on Mass Storage Systems and Technologies (MSST)}, 
  title={The Hadoop Distributed File System}, 
  year={2010},
  volume={},
  number={},
  pages={1-10},
  keywords={File systems;Bandwidth;Concurrent computing;Distributed computing;Computer architecture;File servers;Facebook;Protocols;Protection;Clustering algorithms;Hadoop;HDFS;distributed file system},
  doi={10.1109/MSST.2010.5496972}},

@article{Oleg-ATC18,
author = {Kolosov, Oleg and Yadgar, Gala and Liram, Matan and Tamo, Itzhak and Barg, Alexander},
title = {On Fault Tolerance, Locality, and Optimality in Locally Repairable Codes},
year = {2020},
issue_date = {May 2020},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {16},
number = {2},
issn = {1553-3077},
url = {https://doi.org/10.1145/3381832},
doi = {10.1145/3381832},
abstract = {Erasure codes in large-scale storage systems allow recovery of data from a failed node. A recently developed class of codes, locally repairable codes (LRCs), offers tradeoffs between storage overhead and repair cost. LRCs facilitate efficient recovery scenarios by adding parity blocks to the system. However, these additional blocks may eventually increase the number of blocks that must be reconstructed. Existing LRCs differ in their use of the parity blocks, in their locality semantics, and in their parameter space. Thus, existing theoretical models cannot directly compare different LRCs to determine which code offers the best recovery performance, and at what cost. We perform the first systematic comparison of existing LRC approaches. We analyze Xorbas, Azure’s LRCs, and Optimal-LRCs in light of two new metrics: average degraded read cost and normalized repair cost. We show the tradeoff between these costs and the code’s fault tolerance, and that different approaches offer different choices in this tradeoff. Our experimental evaluation on a Ceph cluster further demonstrates the different effects of realistic system bottlenecks on the benefit from each LRC approach. Despite these differences, the normalized repair cost metric can reliably identify the LRC approach that would achieve the lowest repair cost in each setup.},
journal = {ACM Trans. Storage},
month = {may},
articleno = {11},
numpages = {32},
keywords = {Erasure codes, local repair}
},

@article{lrc-SaurabhKadekodi-fast23,
author = {Kadekodi, Saurabh and Silas, Shashwat and Clausen, David and Merchant, Arif},
title = {Practical Design Considerations for Wide Locally Recoverable Codes (LRCs)},
year = {2023},
issue_date = {November 2023},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {19},
number = {4},
issn = {1553-3077},
url = {https://doi.org/10.1145/3626198},
doi = {10.1145/3626198},
abstract = {Most of the data in large-scale storage clusters is erasure coded. At exascale, optimizing erasure codes for low storage overhead, efficient reconstruction, and easy deployment is of critical importance. Locally recoverable codes (LRCs) have deservedly gained central importance in this field, because they can balance many of these requirements. In our work, we study wide LRCs; LRCs with large number of blocks per stripe and low storage overhead. These codes are a natural next step for practitioners to unlock higher storage savings, but they come with their own challenges. Of particular interest is their reliability, since wider stripes are prone to more simultaneous failures.We conduct a practically minded analysis of several popular and novel LRCs. We find that wide LRC reliability is a subtle phenomenon that is sensitive to several design choices, some of which are overlooked by theoreticians, and others by practitioners. Based on these insights, we construct novel LRCs called Uniform Cauchy LRCs, which show excellent performance in simulations and a 33\% improvement in reliability on unavailability events observed by a wide LRC deployed in a Google storage cluster. We also show that these codes are easy to deploy in a manner that improves their robustness to common maintenance events. Along the way, we also give a remarkably simple and novel construction of distance-optimal LRCs (other constructions are also known), which may be of interest to theory-minded readers.},
journal = {ACM Trans. Storage},
month = {nov},
articleno = {31},
numpages = {26},
keywords = {Reliability, erasure codes, distributed storage systems}
},

@inproceedings{ransomtag-ccs23,
author = {Ma, Boyang and Yang, Yilin and Li, Jinku and Zhang, Fengwei and Shen, Wenbo and Zhou, Yajin and Ma, Jianfeng},
title = {Travelling the Hypervisor and SSD: A Tag-Based Approach Against Crypto Ransomware with Fine-Grained Data Recovery},
year = {2023},
isbn = {9798400700507},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3576915.3616665},
doi = {10.1145/3576915.3616665},
abstract = {Ransomware has evolved from an economic nuisance to a national security threat nowadays, which poses a significant risk to users. To address this problem, we propose RansomTag, a tag-based approach against crypto ransomware with fine-grained data recovery. Compared to state-of-the-art SSD-based solutions, RansomTag makes progress in three aspects. First, it decouples the ransomware detection functionality from the firmware of the SSD and integrates it into a lightweight hypervisor of Type I. Thus, it can leverage the powerful computing capability of the host system and the rich context information, which is introspected from the operating system, to achieve accurate detection of ransomware attacks and defense against potential targeted attacks on SSD characteristics. Further, RansomTag is readily deployed onto desktop personal computers due to its parapass-through architecture. Second, RansomTag bridges the semantic gap between the hypervisor and the SSD through the tag-based approach proposed by us. Third, RansomTag is able to keep 100\% of the user data overwritten or deleted by ransomware, and restore any single or multiple user files to any versions based on timestamps. To validate our approach, we implement a prototype of RansomTag and collect 3,123 recent ransomware samples to evaluate it. The evaluation results show that our prototype effectively protects user data with minimal scale data backup and acceptable performance overhead. In addition, all the attacked files can be completely restored in fine-grained.},
booktitle = {Proceedings of the 2023 ACM SIGSAC Conference on Computer and Communications Security},
pages = {341–355},
numpages = {15},
keywords = {data recovery, fine-grained, hypervisor, ransomware},
location = {<conf-loc>, <city>Copenhagen</city>, <country>Denmark</country>, </conf-loc>},
series = {CCS '23}
},

@article{ransomtab-ccs23,
  title={RansomSpector: An introspection-based approach to detect crypto ransomware},
  author={Tang, Fei and Ma, Boyang and Li, Jinku and Zhang, Fengwei and Su, Jipeng and Ma, Jianfeng},
  journal={Computers \& Security},
  volume={97},
  pages={101997},
  year={2020},
  publisher={Elsevier}
},

@INPROCEEDINGS{ssdinsider,
  author={Baek, SungHa and Jung, Youngdon and Mohaisen, Aziz and Lee, Sungjin and Nyang, DaeHun},
  booktitle={2018 IEEE 38th International Conference on Distributed Computing Systems (ICDCS)}, 
  title={SSD-Insider: Internal Defense of Solid-State Drive against Ransomware with Perfect Data Recovery}, 
  year={2018},
  volume={},
  number={},
  pages={875-884},
  keywords={Malware;Cryptography;Detectors;Monitoring;Feature extraction;Ransomware;SSD;Firmware;Detection;Recovery},
  doi={10.1109/ICDCS.2018.00089}},

@ARTICLE{ssdassisted,
  author={Baek, Sungha and Jung, Youngdon and Mohaisen, David and Lee, Sungjin and Nyang, DaeHun},
  journal={IEEE Transactions on Computers}, 
  title={SSD-Assisted Ransomware Detection and Data Recovery Techniques}, 
  year={2021},
  volume={70},
  number={10},
  pages={1762-1776},
  keywords={Ransomware;Monitoring;Detection algorithms;Cryptography;Payloads;Ransomware;malware detection;data recovery;flash-based SSDs},
  doi={10.1109/TC.2020.3011214}},

@inproceedings{flushguard,
author = {Huang, Jian and Xu, Jun and Xing, Xinyu and Liu, Peng and Qureshi, Moinuddin K.},
title = {FlashGuard: Leveraging Intrinsic Flash Properties to Defend Against Encryption Ransomware},
year = {2017},
isbn = {9781450349468},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3133956.3134035},
doi = {10.1145/3133956.3134035},
abstract = {Encryption ransomware is a malicious software that stealthily encrypts user files and demands a ransom to provide access to these files. Several prior studies have developed systems to detect ransomware by monitoring the activities that typically occur during a ransomware attack. Unfortunately, by the time the ransomware is detected, some files already undergo encryption and the user is still required to pay a ransom to access those files. Furthermore, ransomware variants can obtain kernel privilege, which allows them to terminate software-based defense systems, such as anti-virus. While periodic backups have been explored as a means to mitigate ransomware, such backups incur storage overheads and are still vulnerable as ransomware can obtain kernel privilege to stop or destroy backups. Ideally, we would like to defend against ransomware without relying on software-based solutions and without incurring the storage overheads of backups. To that end, this paper proposes FlashGuard, a ransomware tolerant Solid State Drive (SSD) which has a firmware-level recovery system that allows quick and effective recovery from encryption ransomware without relying on explicit backups. FlashGuard leverages the observation that the existing SSD already performs out-of-place writes in order to mitigate the long erase latency of flash memories. Therefore, when a page is updated or deleted, the older copy of that page is anyway present in the SSD. FlashGuard slightly modifies the garbage collection mechanism of the SSD to retain the copies of the data encrypted by ransomware and ensure effective data recovery. Our experiments with 1,447 manually labeled ransomware samples show that FlashGuard can efficiently restore files encrypted by ransomware. In addition, we demonstrate that FlashGuard has a negligible impact on the performance and lifetime of the SSD.},
booktitle = {Proceedings of the 2017 ACM SIGSAC Conference on Computer and Communications Security},
pages = {2231–2244},
numpages = {14},
keywords = {solid-state drive, encryption ransomware, data recovery},
location = {Dallas, Texas, USA},
series = {CCS '17}
},

@ARTICLE{contentbased,
  author={Min, Donghyun and Ko, Yungwoo and Walker, Ryan and Lee, Junghee and Kim, Youngjae},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems}, 
  title={A Content-Based Ransomware Detection and Backup Solid-State Drive for Ransomware Defense}, 
  year={2022},
  volume={41},
  number={7},
  pages={2038-2051},
  keywords={Ransomware;Performance evaluation;Entropy;Encryption;Machine learning;Libraries;Engines;Ransomware attack;solid-state drive (SSD);storage security;storage system},
  doi={10.1109/TCAD.2021.3099084}},

@INPROCEEDINGS{ransomblocker,
  author={Park, Jisung and Jung, Youngdon and Won, Jonghoon and Kang, Minji and Lee, Sungjin and Kim, Jihong},
  booktitle={2019 56th ACM/IEEE Design Automation Conference (DAC)}, 
  title={RansomBlocker: a Low-Overhead Ransomware-Proof SSD}, 
  year={2019},
  volume={},
  number={},
  pages={1-6},
  keywords={Ransomware;Entropy;Detection algorithms;Detectors;Encryption;Flash memories},
  doi={}},

@inproceedings{rssd,
author = {Reidys, Benjamin and Liu, Peng and Huang, Jian},
title = {RSSD: defend against ransomware with hardware-isolated network-storage codesign and post-attack analysis},
year = {2022},
isbn = {9781450392051},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3503222.3507773},
doi = {10.1145/3503222.3507773},
abstract = {Encryption ransomware has become a notorious malware. It encrypts user data on storage devices like solid-state drives (SSDs) and demands a ransom to restore data for users. To bypass existing defenses, ransomware would keep evolving and performing new attack models. For instance, we identify and validate three new attacks, including (1) garbage-collection (GC) attack that exploits storage capacity and keeps writing data to trigger GC and force SSDs to release the retained data; (2) timing attack that intentionally slows down the pace of encrypting data and hides its I/O patterns to escape existing defense; (3) trimming attack that utilizes the trim command available in SSDs to physically erase data.  To enhance the robustness of SSDs against these attacks, we propose RSSD, a ransomware-aware SSD. It redesigns the flash management of SSDs for enabling the hardware-assisted logging, which can conservatively retain older versions of user data and received storage operations in time order with low overhead. It also employs hardware-isolated NVMe over Ethernet to expand local storage capacity by transparently offloading the logs to remote cloud/servers in a secure manner. RSSD enables post-attack analysis by building a trusted evidence chain of storage operations to assist the investigation of ransomware attacks. We develop RSSD with a real-world SSD FPGA board. Our evaluation shows that RSSD can defend against new and future ransomware attacks, while introducing negligible performance overhead.},
booktitle = {Proceedings of the 27th ACM International Conference on Architectural Support for Programming Languages and Operating Systems},
pages = {726–739},
numpages = {14},
keywords = {Storage Forensics, Solid-State Drive, Ransomware Attacks and Defenses, NVMe over Fabrics},
location = {Lausanne, Switzerland},
series = {ASPLOS '22}
},

@inproceedings{mimosaftl,
author = {Wang, Peiying and Jia, Shijie and Chen, Bo and Xia, Luning and Liu, Peng},
title = {MimosaFTL: Adding Secure and Practical Ransomware Defense Strategy to Flash Translation Layer},
year = {2019},
isbn = {9781450360999},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3292006.3300041},
doi = {10.1145/3292006.3300041},
abstract = {Ransomware attacks have become prevalent nowadays due to sudden flourish of cryptocurrencies. Most existing defense strategies for ransomware, however, are vulnerable to privileged ransomware who can compromise the operating system and hence any backup data stored locally. The out-of-place-update and the isolation nature of flash memory storage, for the first time, makes it possible to design a defense strategy which is secure against the privileged ransomware. In this work, we propose MimosaFTL, a secure and practical ransomware defense strategy for mobile computing devices equipped with flash memory as external storage. MimosaFTL is secure against the privileged malware by taking advantage of unique characteristics of flash storage. In addition, it is more practical (compared to prior work) for real-world deployments by: 1) incorporating a fine-grained detection scheme which can detect presence of ransomware accurately; and 2) allowing the victim to efficiently restore the infected external storage to the exact point when the malware starts to perform corruption. Experimental evaluation shows that, MimosaFTL can mitigate ransomware attacks effectively with a small negative impact on both I/O performance and lifetime of flash storage.},
booktitle = {Proceedings of the Ninth ACM Conference on Data and Application Security and Privacy},
pages = {327–338},
numpages = {12},
keywords = {ransomware detection, ransomware, mobile devices, flash translation layer, binary search, access patterns},
location = {Richardson, Texas, USA},
series = {CODASPY '19}
},

@misc{ceph,
  title = {(accessed April 3, 2024)}, 
  author = {Ceph} ,
  year = {https://ceph.com/en/}, 
},

@techreport{Gluster,
  title={Glusterfs one storage server to rule them all},
  author={Boyer, Eric B and Broomfield, Matthew C and Perrotti, Terrell A},
  year={2012},
  institution={Los Alamos National Lab.(LANL), Los Alamos, NM (United States)}
},

@inproceedings{Swift,
  title={SWIFT: Software implemented fault tolerance},
  author={Reis, George A and Chang, Jonathan and Vachharajani, Neil and Rangan, Ram and August, David I},
  booktitle={International symposium on Code generation and optimization},
  pages={243--254},
  year={2005},
  organization={IEEE}
},

@misc{google-colossus,
  year =  {{https://cloud.google.com/blog/products/storage-data-transfer/a-peek-behind-colossus-googles-file-system}},
  title ={},
  author = {Colossus},
},

@misc{DAOS,
  title ={},
  author = {DAOS},
  year =  {{https://ethereum.org/en/dao/}},
},

@article{Samsung-MDPI-Electronics,
  title={Understanding the Performance Characteristics of Computational Storage Drives: A Case Study with SmartSSD},
  author={Kim, Hwajung and Yeom, Heon Y and Sung, Hanul},
  journal={Electronics},
  volume={10},
  number={21},
  pages={2617},
  year={2021},
  publisher={MDPI}
},

@ARTICLE{scaleflux,
  author={Liu, Libin and Xu, Hong and Niu, Zhixiong and Li, Jingzong and Zhang, Wei and Wang, Peng and Li, Jiamin and Xue, Jason Chun and Wang, Cong},
  journal={IEEE Transactions on Parallel and Distributed Systems}, 
  title={ScaleFlux: Efficient Stateful Scaling in NFV}, 
  year={2022},
  volume={33},
  number={12},
  pages={4801-4817},
  keywords={Logic gates;Bandwidth;Service level agreements;Packet loss;Computer science;Cloud computing;Wide area networks;Network function virtualization;network load detection;flow bandwidth prediction;stateful scaling;service level agreements},
  doi={10.1109/TPDS.2022.3204209}}


@inproceedings{hotstorage24,
author = {Han, Runzhou and Shi, Chao and Mahmud, Tabassum and Yang, Zeren and Esaulov, Vladislav and Wan, Lipeng and Chen, Yong and Wayda, Jim and Wolf, Matthew and Zheng, Mai},
title = {Revisiting Erasure Codes: A Configuration Perspective},
year = {2024},
isbn = {9798400706301},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3655038.3665951},
doi = {10.1145/3655038.3665951},
abstract = {Erasure coding (EC) plays a crucial role in the fault tolerance of modern distributed storage systems (DSS). Inspired by recent research on storage configuration, we study the configuration sensitivity of EC in real DSS in this paper. We systematically inject faults to trigger EC recovery under various configurations, and measure the impact on recovery time and storage overhead quantitatively. Our results show that configurations may affect the EC recovery time significantly (e.g., up to 426\%). More interestingly, theoretically superior codes may perform worse in DSS under certain configurations. Also, there is a system checking period before EC recovery that accounts for 41\% to 58\% of the overall system recovery time, which has been largely ignored in previous studies. Finally, in terms of storage overhead, EC may introduce 32.3\% to 72.0\% more write amplification (WA) than the theoretical expectation, and we derive a formula to help estimate WA more precisely. Our work suggests the importance of considering the context of real DSS for EC research, and we hope the methodology and findings can contribute to a firmer footing for EC optimization in practice.},
booktitle = {Proceedings of the 16th ACM Workshop on Hot Topics in Storage and File Systems},
pages = {93–100},
numpages = {8},
location = {Santa Clara, CA, USA},
series = {HotStorage '24}
}
